Open Source Software: An Approach to Controlling Usage and Risk in Application Ecosystems

The Open Source Software movement has been growing exponentially for a number of years with no signs of slowing. Driving this growth is the widespread availability of libraries and frameworks that provide many functionalities. Developers are saving time and money incorporating this functionality into their applications resulting in faster more feature-rich releases. Despite the growing success and the advantages that open source software provides, there is a dark side. Due to its community construction and largely unregulated distribution, the majority of open source software contains bugs, vulnerabilities and other issues making it highly susceptible to exploits. The lack of oversight, in general, hinders the quality of this software resulting in a trickle-down effect in the applications that use it. Additionally, developers who use open source tend to arbitrarily download the software into their build systems but rarely keep track of what they have downloaded resulting in an excessive amount of open source software in their applications and in their ecosystem. This paper discusses processes and practices that users of open source software can implement into their environments that can safely track and control the introduction and usage of open source software into their applications, and report on some preliminary results obtained in an industrial context. We conclude by discussing governance issues related to the disciplined use and reuse of open source and areas for further improvements.

==> 4.4-dependency-reference-web-application.tex <==
\subsection{Dependency Reference Web Application}
\label{subsec:SBOM-DB-webapp}
The dependency reference database, as described in the previous section is not truly effective without the capability for developers and others to view and reference the content of the SBOM. A web application becomes necessary for developers and decision-makers to view, update and categorize the dependency information that is in the database. The web application provides an important window into what dependencies are currently in the application ecosystem and which ones are approved for use. 

